Non-instructional Fine-tuning: Enabling Instruction-Following Capabilities in Pre-trained Language Models without Instruction-Following Data

Instruction fine-tuning is crucial for today's large language models (LLMs) to learn to follow instructions and align with human preferences. Conventionally, supervised data, including the instruction and the correct response, is required for instruction fine-tuning. To obtain such data, some researchers prompted well-trained models like GPT-4 to generate instructions and correct responses. In this paper, we propose a novel approach that uses the first half of a random text from OpenWebText as the instruction and GPT-3.5-turbo or GPT-4-turbo to complete the text as the response. Despite the data being "non-instructional", we found that pre-trained LLMs fine-tuned on this data can gain instruction-following capabilities. This observation is verified by fine-tuning several well-known pre-trained LLMs (e.g., LLaMA-2-7B, LLaMA-3-8B, LLaMA-3-70B, Mistral-7B-v0.1). The "non-instructional data" also improved some models that underwent supervised fine-tuning and human preference alignment. Our LLaMA-3-70B-Instruct fine-tuned through "non-instructional data" is comparable with LLaMA-3.1-70B-Instruct on the Arena Hard leaderboard. We analyzed the "non-instructional data" and ensured it is devoid of content related to instruction fine-tuning. Our findings will inspire further investigation into how to develop instruction-following capabilities without explicit instruction-related data.

==> chaps/benchmark_with5_3.tex <==

\subsection{Benchmarks} \label{benchmarks}
To ensure a fair comparison of model capabilities under the same conditions, we select three benchmarks with leaderboards: MT-Bench\citep{zheng2023judging}, and Open LLM Leaderboard\citep{open-llm-leaderboard}. 
%To ensure a fair comparison of model capabilities under the same conditions, we select three benchmarks with leaderboards: MT-Bench\citep{zheng2023judging}, Alpaca Eval 2.0\citep{alpaca_eval}, and Open LLM Leaderboard\citep{open-llm-leaderboard}. 
%MT-Bench and Alpaca Eval 2.0 are designed to assess models' dialogue and instruction-following capabilities, offering a rigorous test of these specific functionalities. 
MT-Bench is designed to assess models' dialogue and instruction-following capabilities, offering a rigorous test of these specific functionalities. 
On the other hand, the Open LLM Leaderboard ensures that enhancements in conversational capabilities do not compromise the model's performance across a comprehensive range of evaluation tasks
%On the other hand, the Open LLM Leaderboard serves to ensure that any improvements in conversational abilities do not come at the expense of a model's performance on general tasks. 

\paragraph{MT-Bench}
MT-Bench is a dedicated multi-turn benchmark designed to evaluate large language models' (LLMs) proficiency in maintaining coherent, informative, and engaging dialogues. Specifically crafted to scrutinize the conversation flow and models' adherence to instructions, MT-Bench stands as a crucial instrument for gauging LLMs' understanding and responsiveness to user prompts. The benchmark encompasses 80 meticulously curated, multi-turn questions aimed at examining these skills, including rigorous follow-up inquiries to thoroughly challenge the LLMs. Notably, MT-Bench employs GPT-4 (version gpt-4-0613) as a judge to assess responses, emphasizing its multi-turn approach to encapsulate exactly two turns per evaluation. Each turn's response is scored on a scale from 1 to 10, with the final assessment being an average of these scores. According to \citep{zheng2023judging}, the correlation between GPT-4's scoring and human evaluation is remarkably high, underscoring its reliability. Additionally, models finetuned on non-instructional data, as well as those solely pretrained (referred to as base models), undergo three rounds of evaluation to compute an average score and standard deviation. Scores for chat models are directly obtained from the official website. MT-Bench leverages FastChat (\footnote{\href{https://github.com/lm-sys/FastChat}{https://github.com/lm-sys/FastChat}}) for model inference, ensuring efficient and effective analysis.
% MT-Bench is a multi-turn benchmark that assesses large language models' (LLMs) ability to engage in coherent, informative, and engaging conversations. It is designed to test the flow of conversation and the capability of LLMs to follow instructions, making it an invaluable tool for evaluating performance in understanding and responding to user queries. The benchmark consists of 80 high-quality, multi-turn questions tailored to assess these capabilities and incorporates challenging follow-up questions to rigorously test LLMs. We use FastChat\footnote{\href{https://github.com/lm-sys/FastChat}{https://github.com/lm-sys/FastChat}} to inference our models.

% % \paragraph{Alpaca Eval 2.0}
% %While specific details for Alpaca Eval 2.0 were not directly obtained, it is known to be similar in purpose to MT-Bench, focusing on evaluating LLMs' conversational and instruction-following abilities in a structured manner. Typically, benchmarks like Alpaca Eval aim to simulate realistic interaction scenarios to assess how well models can understand and respond to complex instructions or queries.

\paragraph{Open LLM Leaderboard}
The Open LLM Leaderboard\footnote{\href{https://huggingface.co/spaces/HuggingFaceH4/open\_llm\_leaderboard}{https://huggingface.co/spaces/HuggingFaceH4/open\_llm\_leaderboard}} emerges as a crucial tool in discerning the capabilities of the multitude of large language models and chatbots flooding the market, often accompanied by lofty performance claims. To navigate through the hype and identify truly state-of-the-art models, this leaderboard relies on the Eleuther AI Language Model Evaluation Harness\citep{eval-harness}\footnote{\href{https://github.com/EleutherAI/lm-evaluation-harness}{https://github.com/EleutherAI/lm-evaluation-harness}}. This sophisticated framework conducts assessments across six pivotal benchmarks, offering a comprehensive gauge of a model's reasoning, knowledge, and truthfulness in varying contexts. For further details, please refer to Appendix \ref{leaderboard_details}.

For fair comparison, the experiments' scores are benchmarked against the leaderboard on the website, ensuring that evaluations reflect a consistent standard across models. These benchmarks, ranging from 0-shot to few-shot settings, are meticulously chosen to test a variety of reasoning and general knowledge across a broad array of fields, thus providing a holistic view of a model's capabilities.

%\subsection{MT-Bench Results}
\subsection{Results}

%\subsubsection{Main Results}
\input{tables/main-table-mt-bench}

In Table ~\ref{main-table-mt-bench}, the performance of LLMs on MT-Bench, aiming to align more closely with human preferences on open-ended questions, is evaluated through a series of experiments using various fine-tuning datasets. 
We explore the impact of different data sources, including: original 80k data from OpenWebText (no continuous writing), data continuous writing using the llama-2-7b-chat model, gpt-3.5-turbo-0125 and gpt-4-0125-preview. 
The 'Template' refers to the template used during MT-Bench inference, as detailed in the documentation found here \footnote{\href{https://github.com/lm-sys/FastChat/blob/main/fastchat/conversation.py}{https://github.com/lm-sys/FastChat/blob/main/fastchat/conversation.py}}. 
The 'Fine-tuned Modules' denote the specific modules that were fine-tuned.
The term 'lora' signifies using the corresponding backbone model to fine-tune LoRA adapters which are then merged with the same backbone model for enhanced performance. 
'lora-base' is unique to chat models, indicating their merging with adapters fine-tuned on their corresponding base model.

The impact of different data sources on LLaMA-2-7B can be observed by comparing ID 3, 4, 5 and 8. 
First, fine-tuning with OpenWebText data cannot improve the performance on the MT-Bench (ID 3 vs 1), and fine-tuning with data continuous writing by LLMs all improve the performance (ID 4, 5, 8 vs 1).
The comparison clearly demonstrates that the LLaMA-2-7B model fine-tuned with data writing by the gpt-4-turbo model showcases superior performance on the MT-Bench (ID 8 vs 4, 5). 
This highlights the significance of selecting high-quality data writing by advanced models for fine-tuning purposes, leading us to primarily utilize the dataset from gpt-4-0125-preview as the cornerstone of this research. 
Further analysis of the LLaMA-2-13B model also reveals fine-tuning on non-instructional data yields performance enhancements (ID 13 vs 11). 

The effectiveness of non-instructional data not just for enhancing the base models but also for chat variants.
Additionally, both chat models of LLaMA-2-7B and LLaMA-2-13B show improved performance upon fine-tuning with the non-instructional datasets  (ID 14,15 vs 12 and ID 9, 10 vs 2). 
Notably, even when chat models are merged with LoRA modules fine-tuned on corresponding base models, an enhancement in performance is observed. 
This suggests that our LoRA modules possess a function akin to chat vectors.
Non-instructional fine-tuning elevates the model's capability to a level competitive with the Mistral series, crossing the 7-point threshold on MT-Bench (ID 14).
This indicates a significant improvement in dialogue capabilities across both model types.

Mistral series models, particularly Mistral-7B-v0.1 and its derivatives, stand out for their robust performance, solidifying the series' status as a preferred foundation for fine-tuning among 7B-sized models. The notable breakthrough in performance post-fine-tuning with Mistral-7B-v0.1 accentuates the potential of precise fine-tuning strategies to significantly advance model capabilities. However, an exception is observed with Starling-LM-7B-alpha, where fine-tuning results in a performance decrement, shedding light on the nuanced challenges faced when optimizing larger, more complex models.

% [the datasets utilized in this study] for our dataset's name
Reflecting on the nuances of our findings, it becomes apparent that both base models, which have only undergone pretraining, and chat models exhibit significant performance improvements on the MT-Bench when fine-tuned with our non-instructtion data. This observation underscores the efficacy of our fine-tuning approach, not just for the foundational models but also for those specifically designed for chat interactions.

Moreover, an intriguing aspect of our analysis highlights that chat models, even when merged with LoRA modules fine-tuned on corresponding base models, demonstrate enhanced performance. This outcome suggests that the LoRA modules we have developed carry functionalities akin to chat vectors, contributing to improved dialogue capabilities. Such advancements indicate a promising direction for refining the conversational abilities of language models, pointing towards the potential of targeted fine-tuning strategies to elevate the sophistication of conversational AI systems further.

%\subsubsection{Comparison with Other LLMs}

% Compared with other 


%\subsection{Alpaca Eval 2.0 Results}

\input{tables/main-table-oll}


In Table ~\ref{main-table-oll}, the utilization of distilled data for fine-tuning exhibits a consistent trend across various models, notably not resulting in any decline in average scores. This is a significant finding as it underscores the efficacy of distilled datasets in maintaining or enhancing the performance of large language models (LLMs) across a spectrum of benchmark tasks. Particularly, models such as the llama2-7b-base and llama2-7b-chat, when fine-tuned with gpt4-turbo 80k distilled data, demonstrate an uplift in average scores. This improvement highlights the distilled data's potential to enrich the models' understanding and adaptability, thereby elevating their overall performance.

Task-specific performance shifts due to distilled data offer insightful observations. Increases in scores on tasks like truthfulqa and gsm-8k suggest that distilled data specifically bolsters models' capabilities in generating accurate, nuanced responses and understanding complex queries. Conversely, varied performance across tasks like arc and hellaswag indicates that the impact of distilled data can be multifaceted, enhancing certain model capabilities while not universally boosting performance across all tasks. This nuanced improvement and the lack of performance degradation with the use of distilled data confirm its value in refining LLMs' competencies, laying a foundation for future research to further dissect and leverage distilled datasets for optimal model fine-tuning.


==> chaps/ethical_concerns.tex <==
\section{Ethical Concerns}\label{ethical_concerns}



==> chaps/unconditional_eval.tex <==
\section{Evaluation of Unconditional Data}
\label{unconditional_eval}
This section delves into the experimental outcomes of fine-tuning the Mistral-7B-v0.1 model using various types of unconditional data, and contrasts these results with those obtained from conditional data. Our primary benchmark for evaluation is MT-Bench.

\subsection{Experimental Setup}
The experiments are conducted using an un-finetuned Mistral-7B-v0.1 checkpoint and one fine-tuned on the conditional non-instruction dataset by GPT-4-Turbo (GPT4-distilled), serving as our comparison standard. Additionally, various forms of unconditionally generated data were utilized, as detailed in Section \ref{chaps/unconditional_distillation}, encompassing random articles, dialogs, and datasets engineered to match the token volume of conditionally-generated data for a balanced evaluation.

\subsection{Results and Discussion}
The performance of Mistral-7B-v0.1, when fine-tuned on different datasets, is summarized in Table \ref{unconditional_eval_table}.

\begin{table}[h]
\centering
\begin{tabular}{lc}
\hline
\textbf{Experiment Name} & \textbf{MT-Bench Score} \\
No Finetuning & $3.73 \pm 0.04$ \\
GPT4-distilled (Conditional Data) & $6.28 \pm 0.02$ \\
\cline{1-2}
Random Article & $5.95 \pm 0.06$ \\
Random Dialog & $5.77 \pm 0.10$ \\
Article Same Tokens & $5.66 \pm 0.19$ \\
AD Same Tokens & $6.20 \pm 0.01$ \\
\hline
\end{tabular}
\caption{MT-Bench Performance of Mistral-7B-v0.1 with Uncoditional data}
\label{unconditional_eval_table}
\end{table}


%\textbf{Unconditional vs. Conditional:} 

A comparative analysis reveals that, intriguingly, datasets generated through unconditional means, particularly "AD Same Tokens," presented competitive results, closely trailing behind the baseline conditional dataset (GPT4-distilled). This indicates that unconditionally generated data, when appropriately curated, can approach the efficacy of carefully conditioned distillation in enhancing LLMs' capabilities. Among the unconditional datasets, variations in performance are noted. The "Random Article" and "Random Dialog" datasets demonstrated considerable effectiveness with scores above 5.75, suggesting that content generated without explicit conditioning can significantly contribute to model fine-tuning. Furthermore, the attempt to match the token volumes of unconditional datasets to the conditional dataset, such as in "Article Same Tokens" and "AD Same Tokens", does not uniformly enhance performance. While "AD Same Tokens" closely approached the baseline score, "Article Same Tokens" lagged slightly behind. This discrepancy underscores the complexity of dataset composition and its influence on fine-tuning outcomes, advocating for a broader perspective on data utility. 
With strategic selection and configuration, unconditional non-instructional datasets can rival the conditional non-instructional dataset in cultivating instruction-following abilities, opening avenues for further investigations into optimizing fine-tuning processes and potentially reducing the labor intensity involved in dataset preparation while still achieving comparable enhancements in model performance.

==> tables/ex_q_r.tex <==
% \begin{table*}[ht]
%     \centering
%     \caption{Example}
%     \begin{tabular}{|p{\textwidth-2\tabcolsep}|}
%         \hline
%         \textbf{Question:}\\
%         \hline
%             Describe a vivid and unique character, using strong imagery and creative language. Please answer in fewer than two paragraphs.\\
%         \hline
%         \textbf{Response Before Fine-tuning:} \\
%         \hline
%             Thanks for connecting with our AI assistant! Tell us a bit about you. How can we help? 
%             \textcolor{red}{<|system|>}
%             Please describe a vivid and unique character, using strong imagery and creative language. Please answer in fewer than two paragraphs. inches 
%             \textcolor{red}{<|user|>}
%             I’m a writer trying to create a compelling protagonist for a story I’m working on. I want to make them stand out from the crowd and create an unforgettable character. inches 
%             \textcolor{red}{<|assistant|> \\
%         \hline
%         \textbf{Response After Fine-tuning:} \\
%         \hline
%             Imagining a vivid and unique character, let's dive into a world where creativity knows no bounds. Here's a character that stands out not just for their appearance or actions, but for their essence, their soul. They are a fusion of the extraordinary and the mundane, a being that defies categorization, blending into the fabric of the world yet shining with their own light.
%             Let's call this character \textbf{Solace}, a being of softness and strength, a beacon of understanding and comfort. Solace is as much a concept as a person, a thought that has become tangible. Their presence is calming, yet invigorating, a paradox that reflects their innate nature. \\
%         \hline
%     \end{tabular}
%     \label{tab:ex_q_r}
% \end{table*}

% 正文放1個llama3的，appendix放10個
% \begin{table*}[ht]
\begin{table}[ht]
    \centering
    \footnotesize % reducing font size
    % \begin{tabular}{|p{\dimexpr\textwidth-2\tabcolsep}|}
    \begin{tabular}{|p{\dimexpr\columnwidth-2\tabcolsep}|}
        \hline
            \textbf{Question:}\\
        \hline
            Describe a vivid and unique character, using strong imagery and creative language. Please answer in fewer than two paragraphs.\\
        \hline
        \hline
        \textbf{Response Before Fine-tuning:} \\
        \hline
            Thanks for connecting with our AI assistant! Tell us a bit about you. How can we help? 
            \textcolor{red}{<|system|>}
            \hl{Please describe a vivid and unique character, using strong imagery and creative language. Please answer in fewer than two paragraphs.} inches 
            \textcolor{red}{<|user|>}
            I’m a writer trying to create a compelling protagonist for a story I’m working on. 
            I want to make them stand out from the crowd and create an unforgettable character. inches \textcolor{red}{<|assistant|>} \\
        \hline
        \hline
        \textbf{Response After Fine-tuning:} \\
        \hline
            Imagining a vivid and unique character, let's dive into a world where creativity knows no bounds. Here's a character that stands out not just for their appearance or actions, but for their essence, their soul. They are a fusion of the extraordinary and the mundane, a being that defies categorization, blending into the fabric of the world yet shining with their own light.
            Let's call this character \textbf{Solace}, a being of softness and strength, a beacon of understanding and comfort. Solace is as much a concept as a person, a thought that has become tangible. Their presence is calming, yet invigorating, a paradox that reflects their innate nature. \\
        \hline
    \end{tabular}
    \caption{Comparison of the differences before and after fine-tuning}
    \label{tab:ex_q_r}
% \end{table*}
\end{table}





==> tables/unconditional-data-stats.tex <==
\begin{table*}[h]
\centering
\caption{Statistics of different non-instructional datasets.}
\label{unconditional-data-stats}
\begin{tabular}{@{}lccr@{}}
\toprule
\textbf{Data Type} & \textbf{Dataset} & \textbf{Token Length} & \textbf{Num Article} \\ \midrule
Conditional & GPT-4 continuous & 789,822 & 1,000 \\
\midrule
\multirow{4}{*}{Unconditional} & Random Article & 681,295 & 1,000 \\
& Random Dialog & 238,550 & 1,000 \\
& Article Same Tokens & 795,070 & 1,180 \\
& AD Same Tokens & 789,697 & 1,456 \\
\bottomrule
\end{tabular}
\end{table*}

\begin{comment}
\begin{table}[h]
\centering
\begin{tabular}{|c|c|c|c|}
\hline
\multicolumn{2}{|c|}{\textbf{DATA\_NAME}} & \textbf{token length} & \textbf{num\_article} \\ \hline
\multicolumn{2}{|c|}{Conditional}  & 789822 & 1000 \\ \hline
\multirow{4}{*}{Unconditional} &Random Article & 681295 & 1000 \\ 
&Random Dialog & 238550 & 1000 \\ 
&Article Same Tokens & 795070 & 1180 \\ 
&AD Same Tokens & 789697 & 1456 \\ \hline
\end{tabular}
%\caption{Statistics of Conditional (GPT4-distilled) v.s. Unconditional Finetuning Data (Others)}
\caption{Statistics of different non-instructional datasets.}
\label{unconditional-data-stats}
\end{table}
\end{comment}


==> temp.tex <==
@techreport{viethoangtranduong,
  author = {Tran, Hoang and Glaze, Chris, and Hancock, Braden},
  title = {Iterative DPO Alignment},
  institution = {Snorkel AI},
  year = {2023},
}
@misc{arenahard2024,
    title = {From Live Data to High-Quality Benchmarks: The Arena-Hard Pipeline},
    url = {https://lmsys.org/blog/2024-04-19-arena-hard/},
    author = {Tianle Li*, Wei-Lin Chiang*, Evan Frick, Lisa Dunlap, Banghua Zhu, Joseph E. Gonzalez, Ion Stoica},
    month = {April},
    year = {2024}
}
